TasteRoute: Personalized Routing for Video Generation

Rapid progress in video generation has led to a plethora of models that differ substantially in capability and generation cost. This raises a natural question: can each request be efficiently routed to an appropriate model? We find that even when the consensus of the other annotators is used as an oracle, it agrees with each annotator's own favorite only 34-55% of the time. Motivated by this observation, we introduce TasteRoute, a personalized video-generation router that selects a generator jointly based on the input request, user preferences, and available generation budget. Across text-to-video and image-to-video settings, TasteRoute is competitive with strong simple baselines on preference routing while reducing average generation cost. The cost saving increases under higher budget caps. Finally, we release TasteRoute-3k, a human-annotated dataset containing multi-model video comparisons, quality judgments, preference rankings, and user-profile signals to facilitate future research on personalized and cost-aware video routing.

==> sections/blocks/blk_i2v.tex <==
\paragraph{Prompt-dependent generator strength in image-to-video.}
Figure~\ref{fig:attribute_generator_i2v} is the I2V counterpart of
Figure~\ref{fig:attribute_generator}. The winner changes on 8 of the 12 attributes, three
more than in T2V, so the prompt-dependence that motivates routing is not specific to the
text-to-video setting.

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.66\textwidth]{figures/attribute_generator_i2v.pdf}
  \caption{\textbf{Generator strength depends on the prompt (I2V).} The I2V half of
  Figure~\ref{fig:attribute_generator}, on the same twelve attributes and with the same
  estimator, with numbers only in the mean row. The winner changes on 8 of the 12
  attributes, mostly between the two Veo variants; on-screen text moves every generator
  at once ($-12$ to $-14$ on average, $-31$ for Vidu~Q3~Turbo).}
  \label{fig:attribute_generator_i2v}
\end{figure}

